ForecastPFN: Synthetically-Trained Zero-Shot Forecasting

The vast majority of time-series forecasting approaches require a substantial training dataset. However, many real-life forecasting applications have very little initial observations, sometimes just 40 or fewer. Thus, the applicability of most forecasting methods is restricted in data-sparse commercial applications. While there is recent work in the setting of very limited initial data (so-called `zero-shot' forecasting), its performance is inconsistent depending on the data used for pretraining. In this work, we take a different approach and devise ForecastPFN, the first zero-shot forecasting model trained purely on a novel synthetic data distribution. ForecastPFN is a prior-data fitted network, trained to approximate Bayesian inference, which can make predictions on a new time series dataset in a single forward pass. Through extensive experiments, we show that zero-shot predictions made by ForecastPFN are more accurate and faster compared to state-of-the-art forecasting methods, even when the other methods are allowed to train on hundreds of additional in-distribution data points.

==> table.tex <==
\newcommand\boldblue[1]{\textcolor{blue}{\textbf{#1}}}

\begin{table*}[t]
\centering
\caption{Forecasting results on Illness and Exchange datasets with two budgets, 1 second and 1 minute, for training. A lower MSE indicates better performance. A blue bold is for the best performance on 1 second budget, and black bold is for the best performance on 1 minute budget. Configurations which took twice than their budget to converge are omitted from this table.}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Datasets}&\multicolumn{4}{c|}{Illness}&\multicolumn{4}{c}{Exchange}\\
\midrule
Methods & Budget & 24 & 36 & 48 & 60 & 96 & 192 & 336 & 720\\
\midrule
\multirow{2}{*}{ForecastPFN} & 1s  &  \boldblue{1.011} &  \boldblue{0.799} &  \boldblue{0.881} &  \boldblue{1.047} &    \boldblue{0.237} &  \boldblue{0.351} &  \boldblue{0.577} &  1.231 \\
      & 1m &  1.011 &  0.799 &  0.881 &  1.047 &    0.237 &  \bf{0.351} &  \bf{0.577} &  1.231 \\\midrule
\multirow{2}{*}{FEDformer-w} & 1s  &  1.087 &  1.137 &  1.243 &  1.533 &    0.331 &  0.416 &  0.579 &  \boldblue{1.155} \\
      & 1m &  \bf{0.690} &  \bf{0.548} &  \bf{0.662} &  \bf{0.796} &    0.236 &  0.407 &  0.637 &  1.439 \\\midrule
\multirow{2}{*}{Autoformer} & 1s  &  2.042 &  2.291 &  2.188 &  2.124 &    1.697 &  1.136 &  1.684 &  1.951 \\
      & 1m &  0.712 &  0.590 &  0.715 &  0.904 &    \bf{0.227} &  0.664 &  0.900 &  1.171 \\\midrule
\multirow{2}{*}{Informer} & 1s  &  4.586 &  4.036 &  4.177 &  4.289 &    1.256 &  1.092 &  1.471 &  1.800 \\
      & 1m &  5.039 &  4.052 &  4.210 &  4.688 &    0.966 &  1.577 &  3.188 &  1.673 \\\midrule
\multirow{2}{*}{Prophet} & 1s  &  3.439 &  3.384 &  3.321 &  3.345 &    1.303 &  1.309 &  1.328 &  1.379 \\
      & 1m &  3.439 &  3.384 &  3.321 &  3.345 &    1.303 &  1.309 &  1.328 &  1.379 \\ \midrule
\multirow{2}{*}{Arima} & 1s & -- & -- & -- & -- & -- & -- & -- & -- \\
      & 1m &  3.749 &  3.663 &  3.643 &  3.726 &    1.057 &  1.053 &  1.066 &  \bf{1.077} \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-large}
\end{table*}




